Two-photon MINFLUX with doubled localization precision

Achieving localization with molecular precision has been of great interest for extending fluorescence microscopy to nanoscopy. MINFLUX pioneers this transition through point spread function (PSF) engineering, yet its performance is primarily limited by the signal-to-background ratio. Here we demonstrate that applying two-photon excitation to MINFLUX would double its localization precision through PSF engineering by nonlinear effect. Cram\'er-Rao Bound (CRB) is studied as the maximum localization precision, and CRB of two-photon MINFLUX is halved compared to single-photon MINFLUX in all three dimensions. Meanwhile, in order to achieve same localization precision with single-photon MINFLUX, two-photon MINFLUX requires only 1/4 of fluorescence photons, contributing to a possible 4-fold temporal resolution. Benefitted from two-photon excitation, registration-free multicolor nanoscopy and ultrafast color tracking can be achieved. Localization precision of MINFLUX can also be doubled using excitation with second-order Laguerre-Gaussian beams but would suffer from high fluorescence background compared to single-photon and two-photon first-order MINFLUX.

==> 2p-MINFLUX paper/2pMINFLUX_ref.tex <==

@article{hell1994confocal,
	title={Confocal microscopy with an increased detection aperture: type-B 4Pi confocal microscopy},
	author={Hell, Stefan W and Stelzer, Ernst HK and Lindek, Steffen and Cremer, Christoph},
	journal={Optics Letters},
	volume={19},
	number={3},
	pages={222--224},
	year={1994},
	publisher={Optical Society of America}
}

@article{gustafsson1999i5m,
	title={I5M: 3D widefield light microscopy with better than 100nm axial resolution},
	author={Gustafsson, Mats GL and Agard, DA and Sedat, JW and others},
	journal={Journal of Microscopy},
	volume={195},
	number={1},
	pages={10--16},
	year={1999},
	publisher={Citeseer}
}

@article{bewersdorf2006comparison,
	title={Comparison of I5M and 4Pi-microscopy},
	author={Bewersdorf, J and Schmidt, R and Hell, Stefan W},
	journal={Journal of Microscopy},
	volume={222},
	number={2},
	pages={105--117},
	year={2006},
	publisher={Wiley Online Library}
}

@article{pavani2009three,
	title={Three-dimensional, single-molecule fluorescence imaging beyond the diffraction limit by using a double-helix point spread function},
	author={Pavani, Sri Rama Prasanna and Thompson, Michael A and Biteen, Julie S and Lord, Samuel J and Liu, Na and Twieg, Robert J and Piestun, Rafael and Moerner, WE},
	journal={Proceedings of the National Academy of Sciences},
	volume={106},
	number={9},
	pages={2995--2999},
	year={2009},
	publisher={National Acad Sciences}
}

@article{jia2014isotropic,
	title={Isotropic three-dimensional super-resolution imaging with a self-bending point spread function},
	author={Jia, Shu and Vaughan, Joshua C and Zhuang, Xiaowei},
	journal={Nature Photonics},
	volume={8},
	number={4},
	pages={302--306},
	year={2014},
	publisher={Nature Publishing Group}
}

@article{bestvater2002two,
	title={Two-photon fluorescence absorption and emission spectra of dyes relevant for cell imaging},
	author={Bestvater, F and Spiess, E and Stobrawa, G and Hacker, M and Feurer, T and Porwol, T and Berchner-Pfannschmidt, U and Wotzlaw, C and Acker, Helmut},
	journal={Journal of Microscopy},
	volume={208},
	number={2},
	pages={108--115},
	year={2002},
	publisher={Wiley Online Library}
}

@article{mutze2012excitation,
	title={Excitation spectra and brightness optimization of two-photon excited probes},
	author={M{\"u}tze, J{\"o}rg and Iyer, Vijay and Macklin, John J and Colonell, Jennifer and Karsh, Bill and Petr{\'a}{\v{s}}ek, Zden{\v{e}}k and Schwille, Petra and Looger, Loren L and Lavis, Luke D and Harris, Timothy D},
	journal={Biophysical Journal},
	volume={102},
	number={4},
	pages={934--944},
	year={2012},
	publisher={Elsevier}
}

@article{velasco2015absolute,
	title={Absolute two-photon excitation spectra of red and far-red fluorescent probes},
	author={Velasco, Mary Grace M and Allgeyer, Edward S and Yuan, Peng and Grutzendler, Jaime and Bewersdorf, Joerg},
	journal={Optics Letters},
	volume={40},
	number={21},
	pages={4915--4918},
	year={2015},
	publisher={Optical Society of America}
}

@article{xu2015multiphoton,
	title={Multiphoton excitation of fluorescent probes},
	author={Xu, Chris and Zipfel, Warren R},
	journal={Cold Spring Harbor Protocols},
	volume={2015},
	number={3},
	pages={pdb--top086116},
	year={2015},
	publisher={Cold Spring Harbor Laboratory Press}
}

@article{hell1994breaking,
	title={Breaking the diffraction resolution limit by stimulated emission: stimulated-emission-depletion fluorescence microscopy},
	author={Hell, Stefan W and Wichmann, Jan},
	journal={Optics Letters},
	volume={19},
	number={11},
	pages={780--782},
	year={1994},
	publisher={Optical Society of America}
}

@article{betzig2006imaging,
	title={Imaging intracellular fluorescent proteins at nanometer resolution},
	author={Betzig, Eric and Patterson, George H and Sougrat, Rachid and Lindwasser, O Wolf and Olenych, Scott and Bonifacino, Juan S and Davidson, Michael W and Lippincott-Schwartz, Jennifer and Hess, Harald F},
	journal={Science},
	volume={313},
	number={5793},
	pages={1642--1645},
	year={2006},
	publisher={American Association for the Advancement of Science}
}

@article{2006Stochastic,
	title={Stochastic optical reconstruction microscopy (STORM) provides sub-diffraction-limit image resolution},
	author={ Rust, M. J.  and  Bates, M.  and  Zhuang, X. },
	journal={Nature Methods},
	volume={3},
	number={10},
	pages={793},
	year={2006},
}

@article{balzarotti2017nanometer,
  title={Nanometer resolution imaging and tracking of fluorescent molecules with minimal photon fluxes},
  author={Balzarotti, Francisco and Eilers, Yvan and Gwosch, Klaus C and Gynn{\aa}, Arvid H and Westphal, Volker and Stefani, Fernando D and Elf, Johan and Hell, Stefan W},
  journal={Science},
  volume={355},
  number={6325},
  pages={606--612},
  year={2017},
  publisher={American Association for the Advancement of Science}
}


@article{gwosch2020minflux,
  title={MINFLUX nanoscopy delivers 3D multicolor nanometer resolution in cells},
  author={Gwosch, Klaus C and Pape, Jasmin K and Balzarotti, Francisco and Hoess, Philipp and Ellenberg, Jan and Ries, Jonas and Hell, Stefan W},
  journal={Nature Methods},
  volume={17},
  number={2},
  pages={217--224},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{eilers2018minflux,
  title={MINFLUX monitors rapid molecular jumps with superior spatiotemporal resolution},
  author={Eilers, Yvan and Ta, Haisen and Gwosch, Klaus C and Balzarotti, Francisco and Hell, Stefan W},
  journal={Proceedings of the National Academy of Sciences},
  volume={115},
  number={24},
  pages={6117--6122},
  year={2018},
  publisher={National Acad Sciences}
}

@article{xiao2017flipping,
	title={Flipping nanoscopy on its head},
	author={Xiao, Jie and Ha, Taekjip},
	journal={Science},
	volume={355},
	number={6325},
	pages={582--584},
	year={2017},
	publisher={American Association for the Advancement of Science}
}

@article{roy2008practical,
  title={A practical guide to single-molecule FRET},
  author={Roy, Rahul and Hohng, Sungchul and Ha, Taekjip},
  journal={Nature Methods},
  volume={5},
  number={6},
  pages={507--516},
  year={2008},
  publisher={Nature Publishing Group}
}

@article{ha1996probing,
  title={Probing the interaction between two single molecules: fluorescence resonance energy transfer between a single donor and a single acceptor},
  author={Ha, Taekjip and Enderle, Thilo and Ogletree, DF and Chemla, Daniel S and Selvin, Paul R and Weiss, Shimon},
  journal={Proceedings of the National Academy of Sciences},
  volume={93},
  number={13},
  pages={6264--6268},
  year={1996},
  publisher={National Acad Sciences}
}

@article{wildanger2008sted,
  title={STED microscopy with a supercontinuum laser source},
  author={Wildanger, Dominik and Rittweger, Eva and Kastrup, Lars and Hell, Stefan W},
  journal={Optics Express},
  volume={16},
  number={13},
  pages={9614--9621},
  year={2008},
  publisher={Optical Society of America}
}

@article{pape2020multicolor,
  title={Multicolor 3D MINFLUX nanoscopy of mitochondrial MICOS proteins},
  author={Pape, Jasmin K and Stephan, Till and Balzarotti, Francisco and B{\"u}chner, Rebecca and Lange, Felix and Riedel, Dietmar and Jakobs, Stefan and Hell, Stefan W},
  journal={Proceedings of the National Academy of Sciences},
  volume={117},
  number={34},
  pages={20607--20614},
  year={2020},
  publisher={National Acad Sciences}
}

@article{peticolas1963double,
	title={Double photon excitation in organic crystals},
	author={Peticolas, Warner L and Goldsborough, John P and Rieckhoff, KE},
	journal={Physical Review Letters},
	volume={10},
	number={2},
	pages={43},
	year={1963},
	publisher={APS}
}

@article{sheppard1990image,
	title={Image formation in two-photon fluorescence microscopy},
	author={Sheppard, CJ R and Gu, Min},
	journal={Optik (Stuttgart)},
	volume={86},
	number={3},
	pages={104--106},
	year={1990}
}

@article{denk1990two,
	title={Two-photon laser scanning fluorescence microscopy},
	author={Denk, Winfried and Strickler, James H and Webb, Watt W},
	journal={Science},
	volume={248},
	number={4951},
	pages={73--76},
	year={1990},
	publisher={American Association for the Advancement of Science}
}

@incollection{denk2006multi,
	title={Multi-photon molecular excitation in laser-scanning microscopy},
	author={Denk, Winfried and Piston, David W and Webb, Watt W},
	booktitle={Handbook of Biological Confocal Microscopy},
	pages={535--549},
	year={2006},
	publisher={Springer}
}

@article{harke2008resolution,
	title={Resolution scaling in STED microscopy},
	author={Harke, Benjamin and Keller, Jan and Ullal, Chaitanya K and Westphal, Volker and Sch{\"o}nle, Andreas and Hell, Stefan W},
	journal={Optics Express},
	volume={16},
	number={6},
	pages={4154--4162},
	year={2008},
	publisher={Optical Society of America}
}


@article{wolf1959electromagnetic,
	title={Electromagnetic diffraction in optical systems-I. An integral representation of the image field},
	author={Wolf, Emil},
	journal={Proceedings of the Royal Society of London. Series A. Mathematical and Physical Sciences},
	volume={253},
	number={1274},
	pages={349--357},
	year={1959},
	publisher={The Royal Society London}
}

@article{richards1959electromagnetic,
	title={Electromagnetic diffraction in optical systems, II. Structure of the image field in an aplanatic system},
	author={Richards, Bernard and Wolf, Emil},
	journal={Proceedings of the Royal Society of London. Series A. Mathematical and Physical Sciences},
	volume={253},
	number={1274},
	pages={358--379},
	year={1959},
	publisher={The Royal Society London}
}


@article{xie2013analytical,
	title={Analytical description of high-aperture STED resolution with 0--2$\pi$ vortex phase modulation},
	author={Xie, Hao and Liu, Yujia and Jin, Dayong and Santangelo, Philip J and Xi, Peng},
	journal={JOSA A},
	volume={30},
	number={8},
	pages={1640--1645},
	year={2013},
	publisher={Optical Society of America}
}

@article{backlund2018fundamental,
	title={Fundamental precision bounds for three-dimensional optical localization microscopy with Poisson statistics},
	author={Backlund, Mikael P and Shechtman, Yoav and Walsworth, Ronald L},
	journal={Physical Review Letters},
	volume={121},
	number={2},
	pages={023904},
	year={2018},
	publisher={APS}
}


@article{zhao2007spin,
	title={Spin-to-orbital angular momentum conversion in a strongly focused optical beam},
	author={Zhao, Yiqiong and Edgar, J Scott and Jeffries, Gavin DM and McGloin, David and Chiu, Daniel T},
	journal={Physical Review Letters},
	volume={99},
	number={7},
	pages={073901},
	year={2007},
	publisher={APS}
}

@article{zhan2006properties,
	title={Properties of circularly polarized vortex beams},
	author={Zhan, Qiwen},
	journal={Optics Letters},
	volume={31},
	number={7},
	pages={867--869},
	year={2006},
	publisher={Optical Society of America}
}



@article{youngworth2000focusing,
	title={Focusing of high numerical aperture cylindrical-vector beams},
	author={Youngworth, Kathleen S and Brown, Thomas G},
	journal={Optics Express},
	volume={7},
	number={2},
	pages={77--87},
	year={2000},
	publisher={Optical Society of America}
}



==> 2pMINFLUX_ref.tex <==

@article{hell1994confocal,
	title={Confocal microscopy with an increased detection aperture: type-B 4Pi confocal microscopy},
	author={Hell, Stefan W and Stelzer, Ernst HK and Lindek, Steffen and Cremer, Christoph},
	journal={Optics Letters},
	volume={19},
	number={3},
	pages={222--224},
	year={1994},
	publisher={Optical Society of America}
}

@article{gustafsson1999i5m,
	title={I5M: 3D widefield light microscopy with better than 100nm axial resolution},
	author={Gustafsson, Mats GL and Agard, DA and Sedat, JW and others},
	journal={Journal of Microscopy},
	volume={195},
	number={1},
	pages={10--16},
	year={1999},
	publisher={Citeseer}
}

@article{bewersdorf2006comparison,
	title={Comparison of I5M and 4Pi-microscopy},
	author={Bewersdorf, J and Schmidt, R and Hell, Stefan W},
	journal={Journal of Microscopy},
	volume={222},
	number={2},
	pages={105--117},
	year={2006},
	publisher={Wiley Online Library}
}

@article{pavani2009three,
	title={Three-dimensional, single-molecule fluorescence imaging beyond the diffraction limit by using a double-helix point spread function},
	author={Pavani, Sri Rama Prasanna and Thompson, Michael A and Biteen, Julie S and Lord, Samuel J and Liu, Na and Twieg, Robert J and Piestun, Rafael and Moerner, WE},
	journal={Proceedings of the National Academy of Sciences},
	volume={106},
	number={9},
	pages={2995--2999},
	year={2009},
	publisher={National Acad Sciences}
}

@article{jia2014isotropic,
	title={Isotropic three-dimensional super-resolution imaging with a self-bending point spread function},
	author={Jia, Shu and Vaughan, Joshua C and Zhuang, Xiaowei},
	journal={Nature Photonics},
	volume={8},
	number={4},
	pages={302--306},
	year={2014},
	publisher={Nature Publishing Group}
}

@article{bestvater2002two,
	title={Two-photon fluorescence absorption and emission spectra of dyes relevant for cell imaging},
	author={Bestvater, F and Spiess, E and Stobrawa, G and Hacker, M and Feurer, T and Porwol, T and Berchner-Pfannschmidt, U and Wotzlaw, C and Acker, Helmut},
	journal={Journal of Microscopy},
	volume={208},
	number={2},
	pages={108--115},
	year={2002},
	publisher={Wiley Online Library}
}

@article{mutze2012excitation,
	title={Excitation spectra and brightness optimization of two-photon excited probes},
	author={M{\"u}tze, J{\"o}rg and Iyer, Vijay and Macklin, John J and Colonell, Jennifer and Karsh, Bill and Petr{\'a}{\v{s}}ek, Zden{\v{e}}k and Schwille, Petra and Looger, Loren L and Lavis, Luke D and Harris, Timothy D},
	journal={Biophysical Journal},
	volume={102},
	number={4},
	pages={934--944},
	year={2012},
	publisher={Elsevier}
}

@article{velasco2015absolute,
	title={Absolute two-photon excitation spectra of red and far-red fluorescent probes},
	author={Velasco, Mary Grace M and Allgeyer, Edward S and Yuan, Peng and Grutzendler, Jaime and Bewersdorf, Joerg},
	journal={Optics Letters},
	volume={40},
	number={21},
	pages={4915--4918},
	year={2015},
	publisher={Optical Society of America}
}

@article{xu2015multiphoton,
	title={Multiphoton excitation of fluorescent probes},
	author={Xu, Chris and Zipfel, Warren R},
	journal={Cold Spring Harbor Protocols},
	volume={2015},
	number={3},
	pages={pdb--top086116},
	year={2015},
	publisher={Cold Spring Harbor Laboratory Press}
}

@article{hell1994breaking,
	title={Breaking the diffraction resolution limit by stimulated emission: stimulated-emission-depletion fluorescence microscopy},
	author={Hell, Stefan W and Wichmann, Jan},
	journal={Optics Letters},
	volume={19},
	number={11},
	pages={780--782},
	year={1994},
	publisher={Optical Society of America}
}

@article{betzig2006imaging,
	title={Imaging intracellular fluorescent proteins at nanometer resolution},
	author={Betzig, Eric and Patterson, George H and Sougrat, Rachid and Lindwasser, O Wolf and Olenych, Scott and Bonifacino, Juan S and Davidson, Michael W and Lippincott-Schwartz, Jennifer and Hess, Harald F},
	journal={Science},
	volume={313},
	number={5793},
	pages={1642--1645},
	year={2006},
	publisher={American Association for the Advancement of Science}
}

@article{2006Stochastic,
	title={Stochastic optical reconstruction microscopy (STORM) provides sub-diffraction-limit image resolution},
	author={ Rust, M. J.  and  Bates, M.  and  Zhuang, X. },
	journal={Nature Methods},
	volume={3},
	number={10},
	pages={793},
	year={2006},
}

@article{balzarotti2017nanometer,
  title={Nanometer resolution imaging and tracking of fluorescent molecules with minimal photon fluxes},
  author={Balzarotti, Francisco and Eilers, Yvan and Gwosch, Klaus C and Gynn{\aa}, Arvid H and Westphal, Volker and Stefani, Fernando D and Elf, Johan and Hell, Stefan W},
  journal={Science},
  volume={355},
  number={6325},
  pages={606--612},
  year={2017},
  publisher={American Association for the Advancement of Science}
}


@article{gwosch2020minflux,
  title={MINFLUX nanoscopy delivers 3D multicolor nanometer resolution in cells},
  author={Gwosch, Klaus C and Pape, Jasmin K and Balzarotti, Francisco and Hoess, Philipp and Ellenberg, Jan and Ries, Jonas and Hell, Stefan W},
  journal={Nature Methods},
  volume={17},
  number={2},
  pages={217--224},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{eilers2018minflux,
  title={MINFLUX monitors rapid molecular jumps with superior spatiotemporal resolution},
  author={Eilers, Yvan and Ta, Haisen and Gwosch, Klaus C and Balzarotti, Francisco and Hell, Stefan W},
  journal={Proceedings of the National Academy of Sciences},
  volume={115},
  number={24},
  pages={6117--6122},
  year={2018},
  publisher={National Acad Sciences}
}

@article{xiao2017flipping,
	title={Flipping nanoscopy on its head},
	author={Xiao, Jie and Ha, Taekjip},
	journal={Science},
	volume={355},
	number={6325},
	pages={582--584},
	year={2017},
	publisher={American Association for the Advancement of Science}
}

@article{roy2008practical,
  title={A practical guide to single-molecule FRET},
  author={Roy, Rahul and Hohng, Sungchul and Ha, Taekjip},
  journal={Nature Methods},
  volume={5},
  number={6},
  pages={507--516},
  year={2008},
  publisher={Nature Publishing Group}
}

@article{ha1996probing,
  title={Probing the interaction between two single molecules: fluorescence resonance energy transfer between a single donor and a single acceptor},
  author={Ha, Taekjip and Enderle, Thilo and Ogletree, DF and Chemla, Daniel S and Selvin, Paul R and Weiss, Shimon},
  journal={Proceedings of the National Academy of Sciences},
  volume={93},
  number={13},
  pages={6264--6268},
  year={1996},
  publisher={National Acad Sciences}
}

@article{wildanger2008sted,
  title={STED microscopy with a supercontinuum laser source},
  author={Wildanger, Dominik and Rittweger, Eva and Kastrup, Lars and Hell, Stefan W},
  journal={Optics Express},
  volume={16},
  number={13},
  pages={9614--9621},
  year={2008},
  publisher={Optical Society of America}
}

@article{pape2020multicolor,
  title={Multicolor 3D MINFLUX nanoscopy of mitochondrial MICOS proteins},
  author={Pape, Jasmin K and Stephan, Till and Balzarotti, Francisco and B{\"u}chner, Rebecca and Lange, Felix and Riedel, Dietmar and Jakobs, Stefan and Hell, Stefan W},
  journal={Proceedings of the National Academy of Sciences},
  volume={117},
  number={34},
  pages={20607--20614},
  year={2020},
  publisher={National Acad Sciences}
}

@article{peticolas1963double,
	title={Double photon excitation in organic crystals},
	author={Peticolas, Warner L and Goldsborough, John P and Rieckhoff, KE},
	journal={Physical Review Letters},
	volume={10},
	number={2},
	pages={43},
	year={1963},
	publisher={APS}
}

@article{sheppard1990image,
	title={Image formation in two-photon fluorescence microscopy},
	author={Sheppard, CJ R and Gu, Min},
	journal={Optik (Stuttgart)},
	volume={86},
	number={3},
	pages={104--106},
	year={1990}
}

@article{denk1990two,
	title={Two-photon laser scanning fluorescence microscopy},
	author={Denk, Winfried and Strickler, James H and Webb, Watt W},
	journal={Science},
	volume={248},
	number={4951},
	pages={73--76},
	year={1990},
	publisher={American Association for the Advancement of Science}
}

@incollection{denk2006multi,
	title={Multi-photon molecular excitation in laser-scanning microscopy},
	author={Denk, Winfried and Piston, David W and Webb, Watt W},
	booktitle={Handbook of Biological Confocal Microscopy},
	pages={535--549},
	year={2006},
	publisher={Springer}
}

@article{harke2008resolution,
	title={Resolution scaling in STED microscopy},
	author={Harke, Benjamin and Keller, Jan and Ullal, Chaitanya K and Westphal, Volker and Sch{\"o}nle, Andreas and Hell, Stefan W},
	journal={Optics Express},
	volume={16},
	number={6},
	pages={4154--4162},
	year={2008},
	publisher={Optical Society of America}
}


@article{wolf1959electromagnetic,
	title={Electromagnetic diffraction in optical systems-I. An integral representation of the image field},
	author={Wolf, Emil},
	journal={Proceedings of the Royal Society of London. Series A. Mathematical and Physical Sciences},
	volume={253},
	number={1274},
	pages={349--357},
	year={1959},
	publisher={The Royal Society London}
}

@article{richards1959electromagnetic,
	title={Electromagnetic diffraction in optical systems, II. Structure of the image field in an aplanatic system},
	author={Richards, Bernard and Wolf, Emil},
	journal={Proceedings of the Royal Society of London. Series A. Mathematical and Physical Sciences},
	volume={253},
	number={1274},
	pages={358--379},
	year={1959},
	publisher={The Royal Society London}
}


@article{xie2013analytical,
	title={Analytical description of high-aperture STED resolution with 0--2$\pi$ vortex phase modulation},
	author={Xie, Hao and Liu, Yujia and Jin, Dayong and Santangelo, Philip J and Xi, Peng},
	journal={JOSA A},
	volume={30},
	number={8},
	pages={1640--1645},
	year={2013},
	publisher={Optical Society of America}
}

@article{backlund2018fundamental,
	title={Fundamental precision bounds for three-dimensional optical localization microscopy with Poisson statistics},
	author={Backlund, Mikael P and Shechtman, Yoav and Walsworth, Ronald L},
	journal={Physical Review Letters},
	volume={121},
	number={2},
	pages={023904},
	year={2018},
	publisher={APS}
}


@article{zhao2007spin,
	title={Spin-to-orbital angular momentum conversion in a strongly focused optical beam},
	author={Zhao, Yiqiong and Edgar, J Scott and Jeffries, Gavin DM and McGloin, David and Chiu, Daniel T},
	journal={Physical Review Letters},
	volume={99},
	number={7},
	pages={073901},
	year={2007},
	publisher={APS}
}

@article{zhan2006properties,
	title={Properties of circularly polarized vortex beams},
	author={Zhan, Qiwen},
	journal={Optics Letters},
	volume={31},
	number={7},
	pages={867--869},
	year={2006},
	publisher={Optical Society of America}
}



@article{youngworth2000focusing,
	title={Focusing of high numerical aperture cylindrical-vector beams},
	author={Youngworth, Kathleen S and Brown, Thomas G},
	journal={Optics Express},
	volume={7},
	number={2},
	pages={77--87},
	year={2000},
	publisher={Optical Society of America}
}


